Adversarial Binaries for Authorship Identification

Binary code authorship identification determines authors of a binary program. Existing techniques have used supervised machine learning for this task. In this paper, we look this problem from an attacker's perspective. We aim to modify a test binary, such that it not only causes misprediction but also maintains the functionality of the original input binary. Attacks against binary code are intrinsically more difficult than attacks against domains such as computer vision, where attackers can change each pixel of the input image independently and still maintain a valid image. For binary code, even flipping one bit of a binary may cause the binary to be invalid, to crash at the run-time, or to lose the original functionality. We investigate two types of attacks: untargeted attacks, causing misprediction to any of the incorrect authors, and targeted attacks, causing misprediction to a specific one among the incorrect authors. We develop two key attack capabilities: feature vector modification, generating an adversarial feature vector that both corresponds to a real binary and causes the required misprediction, and input binary modification, modifying the input binary to match the adversarial feature vector while maintaining the functionality of the input binary. We evaluated our attack against classifiers trained with a state-of-the-art method for authorship attribution. The classifiers for authorship identification have 91% accuracy on average. Our untargeted attack has a 96% success rate on average, showing that we can effectively suppress authorship signal. Our targeted attack has a 46% success rate on average, showing that it is possible, but significantly more difficult to impersonate a specific programmer's style. Our attack reveals that existing binary code authorship identification techniques rely on code features that are easy to modify, and thus are vulnerable to attacks.

==> Sections/6-Related.tex <==
\section{Related work}

To the best of our knowledge, there is no existing work on 
evading binary code authorship identification.
The closest was a study conducted by Simko et al. \cite{simko2018recognizing},
with the goal of evading source code single-author identification.

Their evasion target is a classifier
that has 98\% accuracy on classifier 250 authors,
evaluated with the Google Code Jam \cite{Caliskan2015SourceCodeAuthorship}. 
The classifier used lexical features such as variable names and language keywords,
layout features such as code indentation,
and syntactic features derived the abstract syntax trees parsed from the source code.

28 programmers participated their study, 
including undergrad students, former or current software developers.
Each programmer
was given code from author X and Y  
and then was asked to modify source code written by X 
to look like code written by Y.
This manual attack achieved 80\% success rate for untargeted attacks
and 70\% success rate for targeted attacks.

Simko et al. then inspected the modified source code and summarized 
the most common modifications:

\begin{enumerate}
\item Copy entire lines of code written by Y into code written by X;
\item Make typographical changes such as brackets, newlines, space between operators;
\item Modify variable names and the location of variable declarations, typically either from or to a global variable;
\item Add or swap library calls; and
\item Change the source code structure such as adding or removing macros, changing loop types, or breaking up an if-statement
\end{enumerate}

These changes are mostly local, 
involving a few lines of code.
The study participants did not need to understand the structure 
or the functionality of the code to make such modifications.
The modification strategies presented in this study 
are unlikely to achieve equal success for evading 
binary code authorship identification,
as many of the modifications are irrelevant at the binary code level, 
such as typographic changes, variables renaming, and modifying macros.
